Faster Secure Comparisons with Offline Phase for Efficient Private Set Intersection

In a Private section intersection (PSI) protocol, Alice and Bob compute the intersection of their respective sets without disclosing any element not in the intersection. PSI protocols have been extensively studied in the literature and are deployed in industry. With state-of-the-art protocols achieving optimal asymptotic complexity, performance improvements are rare and can only improve complexity constants. In this paper, we present a new private, extremely efficient comparison protocol that leads to a PSI protocol with low constants. A useful property of our comparison protocol is that it can be divided into an online and an offline phase. All expensive cryptographic operations are performed during the offline phase, and the online phase performs only four fast field operations per comparison. This leads to an incredibly fast online phase, and our evaluation shows that it outperforms related work, including KKRT (CCS 16), VOLE-PSI (EuroCrypt 21), and OKVS (Crypto 21). We also evaluate standard approaches to implement the offline phase using different trust assumptions: cryptographic, hardware, and a third party (dealer model).

==> mismatch.tex <==
\section{Label Mismatch}
\label{sec:mismatch}

Let $x_0, \ldots, x_\ell$ be the bit representation of $x$.
Alice uniformly chooses $\ell$ random numbers $r_i$.
If $x_i = 0$ she prepares messages $c_0 = r_i, c_1 = r_i + 1$.
If $x_i = 1$ she prepares messages $c_0 = r_i + 1, c_1 = r_i$.
Alice and Bob engage in an 1-out-of-2 OT where Alice sends $c_0, c_1$ and Bob receives $c_{y_i}$.
Alice computes $e = \sum_{i = 0}^{\ell-1} r_i$.
Bob computes $d = \sum_{i = 0}^{\ell-1} c_{y_i}$ and then $d_{j-1} = d - j$ for $1 \leq j \leq \ell$.
Alice and Bob perform a PSI protocol for $\{ e \}$ and $D = \{ d_0, \ldots, d_{\ell-1} \}$.
If and only if $e \in D$, then $x \neq y$.

In a combined protocol for key value pairs $k_A, X$ and $k_B, y$ there are some optimizations Alice and Bob can do to improve the performance of this abstract construction.
First, we start with $\ell$ modified Beaver triples $r_A, s_{A, i}, r_{B, i}, s_{B, i}$.
Note that $r_A$ is the same across all triples to improve communication efficiency.
Alice computes $r = r_A - H(k_A)$.
She then chooses $\ell - 1$ uniform random numbers $r_i$ for $0 \leq i \leq \ell - 2$ and sets $r_{\ell - 1} = r - \sum_{i = 0}^{\ell-2} r_i$.
Alice and Bob engage in the OT protocols as described above.
Then Bob computes $f_i = (d_i + H(k_B)) r_{B,i} - s_{B, i}$ and sends them back to Alice.
Alice checks if $s_{A,i} \stackrel{?}{=} f_i$ and if it is for any $i$, she concludes that $k_A = k_B$, but $x \neq y$.


==> parameter_estimation.tex <==
beta	log p	no of buckets	log no of buckets	element bit length	MODULUS	bits to compare	Alice to Bob (MB)	Bob to Alice (MB)	Total (MB)	Bits/element online
										
28	-42.88	1,331,692	20.34	12	12,301	14	2.2	62.2	64.5	516
28	-41.88	2,663,383	21.34	11	6,151	13	4.1	115.6	119.7	479
28	-40.88	5,326,766	22.34	10	3,079	12	7.6	213.4	221.0	442
29	-43.49	10,653,532	23.34	9	1,543	11	14.0	405.1	419.1	419
29	-42.49	21,307,064	24.34	8	773	10	25.4	736.6	762.0	381
29	-41.49	42,614,129	25.34	7	389	9	45.7	1,325.9	1,371.6	343
29	-40.49	85,228,257	26.34	6	197	8	81.3	2,357.1	2,438.4	305

==> reduction.tex <==

\section{Reduction of Two-Party Computation to PSI}
\label{sec:reduction}

\begin{table}[!h]
\caption{Intersections $C\cap{}D$ for the different inputs by Alice and Bob.}
\label{tbl:reduction}
\centering
\begin{tabular}{c||c|c|c|c}
\multicolumn{1}{c||}{\multirow{4}{*}{Alice}} & \multicolumn{4}{c}{Bob} \\
\multicolumn{1}{c||}{} & \multicolumn{2}{c|}{$y_0 = 0$} & \multicolumn{2}{c}{$y_1 = 1$} \\
\multicolumn{1}{c||}{} & $y_1 = 0$ & $y_1 = 1$ & $y_1 = 0$ & $y_1 = 1$ \\
\multicolumn{1}{c||}{} & $D = \{2, 3\}$ & $D = \{1, 2\}$ & $D = \{0, 3\}$ & $D = \{0, 1\}$ \\
\hline
\hline
\begin{tabular}{c}
     $b=0$\\
     $C = \{0\}$
\end{tabular}
 & $\emptyset$ & $\emptyset$ & $\{0\}$ & $\{0\}$ \\
\hline
\begin{tabular}{c}
     $b=1$\\
     $C = \{1\}$
\end{tabular}
% $b = 1$ & $C = \{1\}$
& $\emptyset$ & $\{1\}$ & $\emptyset$ & $\{1\}$ \\
\end{tabular}
\end{table}

To underpin the power of PSI, we now present a reduction of two-party computation to PSI.
This reduction may be folklore, but we have not found it spelled out in the literature.
We prove that the existence of one-sided PSI, where only Alice learns the intersection, implies the existence of oblivious transfer (OT) by reducing OT to PSI.
It also proves that public-key operations are necessary for one-sided PSI since they are necessary for oblivious transfer and two-party computation.
The GMW protocol \cite{gmw} over the binary field $\mathbb{Z}_2$ reduces (semi-honest) two-party and multi-party computation to OT.
Reductions of maliciously secure two-party computation also exist \cite{kilian,foundingoteff}.

We compute a 1-out-of-2 OT for one-bit messages.
Alice has $b \in \{ 0, 1 \}$.
Bob has two messages $y_0, y_1 \in \{0, 1\}$.
Alice should obtain $y_{b}$, but not learn anything about $y_{1 - b}$.

If $b = 0$, Alice chooses $C = \{ 0 \}$ as her input set.
If $b = 1$, Alice chooses $C = \{ 1 \}$.
Bob starts by creating an empty set $D$.
If $y_0 = 0$, Bob adds $\{ 2 \}$ to $D$.
If $y_0 = 1$, Bob adds $\{ 0 \}$ to $D$.
If $y_1 = 0$, Bob adds $\{ 3 \}$ to $D$.
If $y_1 = 1$, Bob adds $\{ 1 \}$ to $D$. 

Alice and Bob perform a one-sided PSI protocol for sets $C$ and $D$, such that Alice learns intersection $C\cap{}D$.
Table~\ref{tbl:reduction} shows the resulting intersection.
Observe that the size of input sets is constant ($|C| = 1$, $|D| = 2$).
If the intersection $C\cap{}D$ is empty, then Alice outputs $0$.
If the intersection is either $\{0\}$ or $\{1\}$, Alice outputs $1$.

Note that privately evaluating functions over the intersection is sufficient for this reduction, but not necessary, e.g., set intersection cardinality or set disjointness.
Alice only obtains either of two possible outputs, either the empty set or her input set of size $1$.

Furthermore, OT can be reduced to labelled PSI -- an extended form of PSI.
In labelled PSI Alice obtains a message (label) for her elements in the set.
Bob simply sets the labels $y_i$ for elements $i = \{ 0, 1 \}$.
However, it does not seem obvious how to reduce labelled PSI to PSI which our reduction also implies.


